New $(\alpha,\beta)$ Spanners and Hopsets

An $f(d)$-spanner of an unweighted $n$-vertex graph $G=(V,E)$ is a subgraph $H$ satisfying that $dist_H(u, v)$ is at most $f(dist_G(u, v))$ for every $u,v \in V$. We present new spanner constructions that achieve a nearly optimal stretch of $O(\lceil k /d \rceil)$ for any distance value $d \in [1,k^{1-o(1)}]$, and $d \geq k^{1+o(1)}$. We show the following: 1. There exists an $f(d)$-spanner $H \subseteq G$ with $f(d)\leq 7k$ for any $d \in [1,\sqrt{k}/2]$ with expected size $O_{k}(n^{1+1/k})$. This in particular gives $(\alpha,\beta)$ spanners with $\alpha=O(\sqrt{k})$ and $\beta=O(k)$. 2. For any $\epsilon \in (0,1/2]$, there exists an $(\alpha,\beta)$-spanner with $\alpha=O(k^{\epsilon})$, $\beta=O_{\epsilon}(k)$ and of expected size $O_{k}(n^{1+1/k})$. This implies a stretch of $O(\lceil k/d \rceil)$ for any $d \in [\sqrt{k}/2, k^{1-\epsilon}]$, and for every $d\geq k^{1+\epsilon}$. In particular, it provides a constant stretch already for vertex pairs at distance $k^{1+o(1)}$ (improving upon $d=(\log k)^{\log k}$ that was known before). Up to the $o(1)$ factor in the exponent, and the constant factor in the stretch, this is the best possible by the girth argument. 3. For any $\epsilon \in (0,1)$ and integer $k\geq 1$, there is a $(3+\epsilon, \beta)$-spanner with $\beta=O_{\epsilon}(k^{\log(3+8/\epsilon)})$ and $O_{k,\epsilon}(n^{1+1/k})$ edges. We also consider the related graph concept of hopsets introduced by [Cohen, J. ACM '00]. We present a new family of $(\alpha,\beta)$ hopsets with $\widetilde{O}(k \cdot n^{1+1/k})$ edges and $\alpha \cdot \beta=O(k)$. Most notably, we show a construction of $(3+\epsilon,\beta)$ hopset with $\widetilde{O}_{k,\epsilon}(n^{1+1/k})$ edges and hop-bound of $\beta=O_{\epsilon}(k^{\log(3+9/\epsilon)})$, improving upon the state-of-the-art hop-bound of $\beta=O(\log k /\epsilon)^{\log k}$ by [Elkin-Neiman, '17] and [Huang-Pettie, '17].

==> efficient-spanner.tex <==
\section{Efficient Constructions of $(\alpha,\beta)$ Spanners}
In this section, we provide efficient implementation of $(\alpha,\beta)$ spanners for $\alpha=O(1)$ in various computational settings.

\paragraph{A Modified Meta-Algorithm} 
Optimized variant of our $(\alpha,\beta)$ spanner for the case where $\alpha=3+\epsilon$. For example, we show that a $(4,\beta)$ spanner for $\beta=k^{\log 21}$. Our main result is:
\begin{lemma}\label{lem:3plusepsspanner}
For any $n$-vertex unweighted graph $G=(V,E)$, integer $k$ and constant $\epsilon>0$, one can compute a $(3+\epsilon,\beta)$ spanner $H$ of $G$ for $\beta=O((5+ 16/\epsilon)\cdot k^{\log(5+16/\epsilon)})$ and expected size $|E(H)|=O(n^{1+1/k}+k^{\log(5+16/\epsilon)}\cdot n/\epsilon^2)$.
\end{lemma}
\paragraph{Algorithm Description.}	
For simplicity, we assume throughout that $4/\epsilon$ is an integer. The algorithm contains $T=\lceil \log k +1 \rceil$ clustering phases. Starting with the trivial clustering $\mathcal{C}_{0}= \{\{v\} ~\mid~ v\in V\}$ of radius $0$, in each phase $i\geq 1$, given is a clustering $\mathcal{C}_{i-1}$ of expected size $n_{i-1}=n^{1-\frac{2^{i-2}}{k}}$ (except $i=1$ where $n_{0}=n$) with radius at most $r_{i-1}\le 2\cdot (5+ 16/\epsilon)^{i-1}$. The output of the $i^{th}$ phase is a clustering $\mathcal{C}_i$ of radius $r_i\leq 2\cdot (5+ 16/\epsilon)^{i}$, and a subgraphs $H_i$ that takes care of the unclustered vertices in $V(\mathcal{C}_i)\setminus V(\mathcal{C}_{i-1})$. %For any clustering $\mathcal{C}$, we denote by  $Z(\mathcal{C})$ the set of clusters' centers in $\mathcal{C}$, and for a cluster $C$, we denote its center by $Z(C)$.

We now zoom into $i^{th}$ phase and explain the construction of the clustering $\mathcal{C}_i$, and the subgraph $H_i$. The phase is governed by two key parameters: the sampling probability $p_i$ of each cluster $C \in \mathcal{C}_{i-1}$ to join the clustering $\mathcal{C}_i$, and an augmentation radius $\alpha_i$.
Let $\alpha_1=1/2, p_1=n^{-1/k}$ and for every $i\geq 2$, define
\begin{equation}\label{eq:alpha-p}
\alpha_i = \frac{4}{\epsilon}\cdot r_{i-1} \mbox{~~and~~} p_i=|\mathcal{C}_{i-1}|/n~.
\end{equation}
The description of the $i^{th}$ phase for $i \in \{1,\ldots, T\}$ is as follows:
\begin{enumerate}
\item Each unclustered vertex $v \in V\setminus {V(\mathcal{C}_{i-1})}$ with $\cdist_{G}(v,\mathcal{C}_{i-1})\le r_{i-1}+\alpha_{i}$, adds to $H_{i}$ the shortest path to its closest center in $\mathcal{C}_{i-1}$.
\item Let $\mathcal{C}' \subseteq \mathcal{C}_{i-1}$ be the collection of clusters obtained by 
sampling each cluster $C_\ell \in \mathcal{C}_{i-1}$ independently with probability of $p_i$.
\item Each cluster $C \in \mathcal{C}_{i-1}$ such that $\cdist_{G}(C,\mathcal{C}')\le 4\cdot r_{i-1}+4\cdot \alpha_{i}$, joins the sampled cluster in $\mathcal{C}'$ with minimal distance between their centers, and adds the shortest path between their centers into $H_{i}$.
\item The clustering $\mathcal{C}_{i}$ consists of all the sampled clusters in $\mathcal{C}'$ augmented by their nearby clusters in $\mathcal{C}_{i-1}$ (i.e., at distance $4\cdot r_{i-1}+4\cdot \alpha_{i}$ between their centers). That is, each cluster in $\mathcal{C}_{i}$ is made of star center $C \in \mathcal{C}'$ connected to clusters in $\mathcal{C}_{i-1}$.
\item Each cluster $C \in \mathcal{C}_{i-1}$ such that $\cdist_{G}(C,\mathcal{C}')> 4\cdot r_{i-1}+4\cdot \alpha_{i}$, adds to $H_{i}$ the shortest path between its center to any center of  $C'\in \mathcal{C}_{i-1}$ with $\cdist_{G}(C,C')\le 2\cdot r_{i-1}+2\cdot \alpha_{i}$. 
\end{enumerate}
This completes the description of the $i^{th}$ phase. Let $H=\bigcup_{i=1}^{T} H_i$ and let $\mathcal{C}_T$ be the output clustering of the last phase $T$. In the analysis section we show that in expectation $\mathcal{C}_T$ consists of a single cluster $C$. Finally, the algorithm adds to the output spanner $H$, a BFS tree rooted at the center $z$ of the single cluster $C \in \mathcal{C}_T$. 

\paragraph{Stretch Analysis.}
We start by bounding the radius $r_i$ of the clustering $\mathcal{C}_i$ for every $i \in \{1,\ldots, T\}$.
We first make a simple observation:
\begin{observation}
\label{obs:rad3epsspanner}
For every $i \in \{1,\ldots, T\}$, $r_i \leq 2\cdot (5+ 16/\epsilon)^{i-1}$. In particular, the radius of cluster in the final clustering $\mathcal{C}_T$ is $r_T \le 2\cdot (5+ 16/\epsilon)^{\log{k}+1}=(10+ 32/\epsilon)\cdot k^{\log(5+ 16/\epsilon)}$.
\end{observation}
\begin{proof}
The claim is shown by induction on $i$. For the base case, where $i=1$, the $0$-level clusters are simply nodes, and each node joins the sampled vertex at distance at most $4\cdot r_{0}+4\cdot \alpha_1=2$. Therefore the clusters in $\mathcal{C}_1$ have radius of $2$. Assume that the claim holds up to $i-1 \geq 0$, and consider the $i^{th}$ where the clustering $\mathcal{C}_i$ is defined based on $\mathcal{C}_{i-1}$. Each cluster in  $\mathcal{C}_i$ is formed by a star: the center of the star is the sampled cluster $C$ that is connected to all clusters $C' \in \mathcal{C}_{i-1}$ with center-distance at most $4\cdot r_{i-1}+4\alpha_{i}$ from $C$. The radius of this cluster in $\mathcal{C}_i$ is bounded by
$$r_i \leq r_{i-1}+4\cdot r_{i-1}+4\alpha_{i}= 5\cdot r_{i-1}+16/\epsilon \cdot r_{i-1} \leq 2\cdot \left (5+16/\epsilon \right)^{i-1}~,$$
where the second inequality follows by plugging the bound on $r_{i-1}$ obtained from the induction assumption and the bound on $\alpha_i$ from Eq. (\ref{eq:alpha-p}).
\end{proof}
\begin{observation}
\label{obs:clusters}
For $1\le i \le T$, $\mathbb{E}[|\mathcal{C}_{i}|]=n^{1-2^{i-1}/k}$ therefore after $T$ phases, there is one cluster in $\mathcal{C}_T$ in expectation.
\end{observation}
\begin{proof}
By induction on $i$: for the base case $i=1$, since $p_1=n^{1/k}$, the number of sampled clusters is $n^{1-1/k}$ in expectation. Assume that the claim holds up to $i-1 \geq 1$, and consider the $i^{th}$ clustering. In the $i^{th}$ phase, each cluster in $\mathcal{C}_{i-1}$ is sampled with probability of $p_i=|\mathcal{C}_{i-1}|/n$, there for 
the number of sampled clusters in expectation is $\mathbb{E}[|\mathcal{C}_{i-1}|]^2/n$. By induction assumption, $\mathbb{E}[|\mathcal{C}_{i-1}|]=n^{1-2^{i-2}/k}$, and thus $\mathbb{E}[|\mathcal{C}_{i}|]=n^{1-2^{i-1}/k}$.
By plugging $T=\lceil \log k+1 \rceil$, we get that $\mathbb{E}[|\mathcal{C}_{T}|]=1$.
\end{proof}
Our stretch argument is based on the following definition of clustered vertices.
\begin{definition}
For every $1 \leq i\leq T$, every $v \in V(\mathcal{C}_{i-1})\setminus{V(\mathcal{C}_{i})}$ is called $i$-\emph{unclustered}. In addition, every $v\in V(\mathcal{C}_T)$ is called \emph{clustered} (i.e., $v$ belongs to the final clustering). 
\end{definition}
For every $i$-unclustered vertex we provide a stretch guarantee as a function of $i$. Specifically, the earlier that the vertex $u$ stops being cluster, the smaller is the ball around $u$ for which the stretch guarantee is provided.
\begin{claim}[$1$-unclustered]
\label{cl:1-unc}
For any $1$-unclustered vertex $u\in V$, it holds that $\dist_{H}(u,v) = 1$ for all $v\in N_{G}(u)$.
\end{claim}
\begin{proof}
For the first phase, every $1$-unclustered vertex $u$ adds to the spanner its edges to any vertex at distance $2\alpha_1=1$, the claim follows.
\end{proof}
\begin{claim}[$i$-unclustered]
\label{claim:i-unc}
For any $i$-unclustered vertex $u$ for every $i \in \{2,\ldots, T\}$, and every $v \in \Ball_{G}(u,\alpha_i)$, it holds that $\dist_H(u,v)\leq 3\cdot \dist_{G}(u,v)+4\cdot r_{i-1}$. In particular, for $v \in \partial \Ball_{G}(u,\alpha_i)$, it holds that $\dist_{H}(u,v)\le (3+\epsilon)\cdot \dist_{G}(u,v)$. 
\end{claim}
\begin{proof}
Consider an $i$-unclustered vertex $u$ and $v \in \Ball_{G}(u,\alpha_i)$. By definition, $u \in V(\mathcal{C}_{i-1})$, thus $\cdist_G(v, \mathcal{C}_{i-1})\leq \dist_{G}(v,u)+\cdist_{G}(u,\mathcal{C}_{i-1})\leq r_{i-1}+\alpha_i$. Let $C_v$ be the cluster with the closest center to $v$ in $\mathcal{C}_{i-1}$, and let $C_u$ be the cluster of $u$ in $\mathcal{C}_{i-1}$. Then, the algorithm adds to $H_i$ a shortest path from $v$ to the center of $C_{v}$ of length at most $r_{i-1}+\dist_{G}(u,v)$. We have
\begin{eqnarray*}
\cdist_{G}(C_{u},C_{v})&\le& \cdist_{G}(C_{u},u)+\dist_{G}(u,v)+\cdist_{G}(v,C_{v}) \leq 2\cdot r_{i-1}+ 2\cdot \dist_{G}(u,v)~.
\end{eqnarray*}
Since $C_{u}$ becomes unclustered we add to $H_{i}$ the shortest path between the centers of $C_{u}$ and $C_{v}$.
Overall, we have that
\begin{eqnarray*}
\dist_{H}(u,v)&\le& \cdist_H(u,C_{u})+\cdist_{G}(C_{u},C_{v})+\cdist_{G}(C_{v},v)
\\& \leq & 
r_{i-1}+2\cdot r_{i-1}+ 2\cdot \dist_{G}(u,v)+r_{i-1}+\dist_{G}(u,v)\le 4\cdot r_{i-1}+3\cdot \dist_{G}(u,v)~.
\end{eqnarray*}
\end{proof}
\begin{claim}
\label{claim:clustered3epsspanner}
Let $u,v\in V$ and let $P_{uv}$ be the shortest path between them in $G$. If there is a clustered vertex $w\in P_{uv}$ then $\dist_{H}(u,v)\le \dist_{G}(u,v)+ 2\cdot (10+32/\epsilon)\cdot k^{\log(5+ 16/\epsilon)}$.
\end{claim}
\begin{proof}
Since $w$ is clustered, its distance from the single last cluster center $z$ is at most $r_{T}$. As the algorithm adds the BFS tree of $z$ to the spanner, we have:
\begin{eqnarray*}
\dist_{H}(u,v)&\le& \dist_{H}(u,z)+\dist_{H}(z,v)= \dist_{G}(u,z)+\dist_{G}(z,v)
\\&\le& \dist_{G}(u,w)+\dist_{G}(w,z)+\dist_{G}(z,w)+\dist_{G}(w,v)\le \dist_{G}(u,v)+2\cdot r_{T}~,
\end{eqnarray*}
the claim follows by plugging the bound on $r_T$ from Obs. \ref{obs:rad3epsspanner}.
\end{proof}
We are now ready to complete the stretch argument for Lemma \ref{lem:3plusepsspanner}.
\begin{proof}[Proof of Lemma \ref{lem:3plusepsspanner}]
Let $u,v\in V$ be vertices at some distance\footnote{Unlike the constructions in earlier sections, this construction works for all distances $d$, and there is no need to consider each distance class separately.} $d$ in $G$, and let $P:=\{u:=v_{0},\cdots , v_{d+1}:=v\}$ be the shortest path between them in $G$. First observe that by Claim \ref{claim:clustered3epsspanner}, if there is some clustered vertex in $P$ then we are done. Assume from now on that no vertex on the path is clustered. We define a sequence of vertices between $u$ and $v$ in an iterative manner: let $u_{0}:=u$, and for every $j \in \{1,\ldots, d\}$ given that $u_{j}=v_{i}$, define $u_{j+1}=v_{i+\Delta_{j+1}}$ where: 
\begin{equation*}
\Delta_{j+1}=\begin{cases}
0 & u_{j}=v\\
1 & u_{j}\text{ is \ensuremath{1}-unclustered}\\
\min\{\alpha_\ell,\dist_{G}(u_{j},v)\} & u_{j}\text{ is \ensuremath{\ell\ge 2} unclustered}
\end{cases}
\end{equation*}
Let $\ell'\leq d$ be the first such that $u_{\ell'}=v$, thus we have defined $\ell'-1$ segments $P_{u,v}[u_j,u_{j+1}]$.
%For any segment $j\leq \ell'-2$ of $P_{u,v}[u_j,u_{j+1}]$ it holds that $u_{j+1}\neq v$. Therefore letting $u_j$ be an $\ell$-unclustered vertex, it holds that $u_{j+1} \in N_G(u_j)$ if $u_j$ is $1$-unclustered, and otherwise $u_{j+1} \in \partial \Ball_{G}(u_{j},\alpha_\ell)$. By Claim \ref{cl:1-unc}, in the first case 
By Claim \ref{cl:1-unc}, the second rule causes no stretch. By Claim \ref{claim:i-unc} the third rule causes a maximal stretch of $3+\epsilon$, unless it ends in $v$ which can happen only once, in such a case we get an extra additive term of $4\cdot r_{T-1}\le 8\cdot k^{\log(5+16/\epsilon)}$. Over all we have
\begin{eqnarray*}
\dist_{H}(u,v)&\le&\sum_{j=0}^{\ell'-1}\dist_{H}(u_{j},u_{j+1})\le 4\cdot r_{T-1}+\sum_{j=0}^{d}(3+\epsilon)\cdot \dist_{G}(u_{j},u_{j+1}) 
\\&\le& (3+\epsilon)\cdot \dist_{G}(u,v)+8\cdot k^{\log(5+16/\epsilon)}.
\end{eqnarray*}

\textbf{Size Analysis.}  
At each phase $i \geq 1$ we add the following edges to $H_i$. Each vertex adds a path of length at most $r_{i-1}+\alpha_i$ to its closest cluster center in $\mathcal{C}_{i-1}$. This adds $O(n)$ edges in total by breaking shortest path ties in a consistent manner. The paths that connects clusters in $\mathcal{C}_{i-1}$ to the sampled clusters also consume at most $O(n)$ edges. 
Finally we claim that in the third stage of the $i$th iteration, in which we connect clusters that were not super-clustered to nearby clusters, we add in expectation a small amount of shortest paths:
\begin{lemma}
	\label{lem:expectedamountofsp}
	In the third stage of the $i$th iteration, we add to $H_{i}$ an expected amount of $1/p_{i}$ shortest paths from each cluster.
\end{lemma}
\begin{proof}
	Let $C\in \mathcal{C}_{i-1}$ and let $C_{1}\cdots C_{\ell}$ be the clusters with centers at distance at most $2\cdot r_{i-1}+2\cdot \alpha_{i-1}$ from $C$'s center, ordered by their ID. Note that the centers of each pair of these clusters is at distance at most $4\cdot r_{i-1}+4\cdot \alpha_{i-1}$, thus if one of these clusters is sampled, then all the others would be super-clustered and none would take part in the third stage of the algorithm. Thus in expectation the amount of shortest paths from $C$ added in this stage is $\ell\cdot (1-p_{i})^{\ell}\le 1/p_{i}$. 
\end{proof}
Thus since in this stage there are $|\mathcal{C}_{i-1}|$ clusters and the added shortest paths are of length at most $2\cdot r_{i-1} +2\cdot \alpha_{i}$, we add an expected amount of at most $(2\cdot r_{i-1} +2\cdot \alpha_{i})\cdot |\mathcal{C}_{i-1}|/p_{i}$ edges. Thus $|E(H_{1})|\le n^{1+1/k}+n$ edges, and for $1\le i \le T$,  $|E(H_{i})|\le r_{i}\cdot n$ edges. 
The expected number of edges in union of all the $H_i$ subgraphs for $i \in \{1,\ldots, T\}$ is thus bounded by 
\begin{eqnarray*}
\sum_{i=1}^T |E(H_i)|&\leq & n^{1+1/k}+\sum_{i=2}^{T}r_{i}\cdot n=
n^{1+1/k}+O(n \cdot \sum_{i=2}^{T}(5+ 16/\epsilon)^{i-1})
\\&=&O(n^{1+1/k}+k^{\log(5+16/\epsilon)}\cdot n/\epsilon^2)~.
\end {eqnarray*}
The last stage adds a BFS tree with $n-1$ edges. Lemma \ref{lem:3plusepsspanner} follows.
\end{proof}
\textbf{Running Time.} 
In the analysis of the time complexity we follow \cite{ElkinN19} in introducing a parameter $0<\rho\le 1$ that will allow  freedom in the trade-off between the spanner's size and running time of the algorithm. Specifically, given $\rho$, we define $i_{0}=\lceil \log{(k\cdot \rho)} \rceil$, and $i_{1}=\lceil 2/\rho -1 \rceil$. Now instead of $T$ iterations, we do $i_{0}+i_{1}$ iterations and we redefine the sampling rates, by setting for $1\le i \le i_{0}$ the sampling rate to be $p_{i}$ as defined in Eq. \ref{eq:alpha-p}, and for $i_{0}\le i\le i_{1}$, we fix $p_{i}$ to be $p_{i_{0}}$. The trade-off is summarized in the following Lemma:
\begin{lemma}
	For any graph $G=(V,E)$, integer $k$ and constants $\epsilon>0,1\ge \rho>0$, one can compute a $(3+\epsilon,\beta)$ spanner $H$ of $G$ for $\beta = O((5+16/\epsilon)^{\log{\rho}+2/\rho}\cdot k^{\log(5+16/\epsilon)})$ in $O((\log{(k\cdot \rho)}+1/\rho)\cdot |E|\cdot n^{\rho})$ time.
\end{lemma}
\begin{proof}
	Following the change in the sampling rates, we have $i_{0}+i_{1}=\lceil \log{(k\cdot \rho)} \rceil + \lceil 2/\rho -1 \rceil \le \log(k\cdot \rho)+2/\rho$ iterations. By Observation \ref{obs:rad3epsspanner}, at each iteration we increase the radius by a multiplicative factor of $(5+16/\epsilon)$, thus the radius of the final clustering after these steps would be:
	\begin{eqnarray*}
		r_{i_{0}+i_{1}}\le 2\cdot (5+16/\epsilon)^{i_{0}+i_{1}-1}\le 2\cdot (5+16/\epsilon)^{\log{(k\cdot \rho)}+2/\rho}=2\cdot (5+16/\epsilon)^{\log{\rho}+2/\rho}\cdot k^{\log(5+16/\epsilon)}.
\end{eqnarray*}

In each iteration we do $3$ stages that we would consider in our analysis. The first consists of connecting vertices at distance at most $\alpha_{i}$ from the clustering. The second consists with connecting clusters into super-clusters. The third stage is the one in which we connect unclustered clusters to nearby clusters.
\paragraph{First stage} The first stage consists of running a bounded depth BFS from the clusters' centers to a depth of $r_{i-1}+\alpha_{i}$. This stage can be done in $O(|E|)$-time. The reason is that we can run a 'layered' bounded BFS traversal from all clusters' centers. That is, we order the clusters by their ID, and run an iterative algorithm, such that in the $i$th iteration each cluster center in its turn does its $i$th level BFS-traversal, deleting all edges it traversed so that no edge would be traversed by two clusters. Specifically in the $i$th iteration, when getting to $C$'s turn, we have a subgraph $G'$ containing all the edges that were not traversed yet, and we have $T_{i-1}(C)$, the $i-1$-depth BFS traversal from the center of $C$ had built so far. At this iteration the traversal continues from all the leaves of $T_{i-1}(C)$ to their neighbors in $G'$. When finishing, a new subtree $T_{i}(C)$ is defined to include all the edges of $T_{i-1}(C)$ together with the edges and nodes explored in this iteration. Finally the edges traversed in this iteration are deleted from $E(G')$. After $r_{i-1}+\alpha_{i}$ iterations we halt, adding $\bigcup_{C\in \mathcal{C}_{i-1}}E(T_{r_{i-1}+\alpha_{i}}(C))$ to $H_{i}$. This algorithm is correct since if $v$ is an unclustered vertex at distance at most $r_{i-1}+\alpha_{i}$ from a cluster center, then since we order the clusters by ID, the closest cluster to it would reach it first in its BFS traversal. The algorithm would run in $O(|E|)$ time since no edge would be explored by two different clusters.
\paragraph{Second stage} The second stage consists of running a bounded depth BFS from the sampled clusters' centers to a depth of $4\cdot r_{i-1}+4\cdot \alpha_{i-1}$. This stage can also be done in $O(|E|)$-time by running a 'layered' BFS as in the last stage.
\paragraph{Third stage} The third stage consists of running a bounded depth BFS from the centers of unsampled clusters that were not super-clustered to a depth of $2\cdot r_{i-1}+2\cdot \alpha_{i-1}$. We first claim that any vertex in the graph does not get visited by many BFS traversals:
	\begin{lemma}
		\label{lem:numberofbfstaversals}
		In the third stage of the $i$th iteration, any $v\in V$ is visited by $1/p_{i}$ BFS traversals in expectation.
	\end{lemma}
	\begin{proof}
	The proof of the lemma follows from the proof of Lemma \ref{lem:expectedamountofsp}.
	\end{proof}
	Thus since we have that $p_{i}\ge p_{i_{0}}=n^{-2^{i_{0}-1}/k}\ge n^{-\rho}$, we have that each iteration can be computed in expected time $O(|E|\cdot n^{\rho})$.  
	Over all the expected running time is $O((i_{0}+i_{1})\cdot |E|\cdot n^{\rho})=O((\log{(k\cdot \rho)}+1/\rho)\cdot |E|\cdot n^{\rho})$. 
\end{proof}
\subsection*{Distributed Implementation}
The algorithm translates almost entirely to the distributed setting in a straight forward way. Whenever there is sampling with probability $p_{i}$ in the centralized algorithm, each node of the vertex set we are sampling from would sample itself with probability $p_{i}$, and each bounded-BFS traversal in the algorithm is done in a distributed way. To make the algorithm efficient in the distributed model we need only to change last step, and instead of adding a full BFS traversal from the center of the last cluster, we will do a $5\cdot r_{T}$-depth BFS traversal. This would end with the following $(4+\epsilon)$-stretch hopsets\footnote{Actually $(3+\epsilon+\rho)$-stretch is possible in the \local\ model and $(3+\epsilon+\rho/n^{\rho})$-stretch in the \congest\ with the same round-complexity by enlraging the depth of the last BFS traversal.}:
\begin{lemma}\label{lem:3plusepsspannerloc}
For any graph $G=(V,E)$, integer $k$ and constants $\epsilon>0,1\ge \rho>0$, one can compute in the \local\ model a $(4+\epsilon,\beta)$ spanner $H$ of $G$ for $\beta = O((5+16/\epsilon)^{\log{\rho}+2/\rho}\cdot k^{\log(5+16/\epsilon)})$ in $\widetilde{O}(\beta)$ rounds w.h.p.
\end{lemma}
\begin{lemma}\label{lem:3plusepsspannercongest}
For any graph $G=(V,E)$, integer $k$ and constants $\epsilon>0,1\ge \rho>0$, one can compute in the \congest\ model a $(4+\epsilon,\beta)$ spanner $H$ of $G$ for $\beta = O((5+16/\epsilon)^{\log{\rho}+2/\rho}\cdot k^{\log(5+16/\epsilon)})$ in $\widetilde{O}(n^{\rho}\cdot \beta)$ rounds w.h.p.
\end{lemma}

\begin{proof}
	We begin by proving the stretch argument. Note that we only changed the last step, thus we need only to show that for any $u,v\in V$ such that there is a clustered vertex $w\in V$ on their shortest path in $G$, the algorithm provides good stretch. Indeed:
	\begin{claim}
		For any $u,v\in V$ with shortest path $P$ in $G$, if there is a clustered vertex $w\in V(P)$, then:
		\begin{equation*}
		\dist_{H}(u,v)\le (4+\epsilon)\cdot \dist_{G}(u,v)+O((5+16/\epsilon)^{\log{\rho}+2/\rho}\cdot k^{\log(5+16/\epsilon)})
		\end{equation*}
	\end{claim} 
	\begin{proof}
		First note that if $\dist_{G}(u,v)\le 4\cdot r_{T}$, then in the last step of the algorithm we would add a shortest path between $u$ and $v$ to the center of the cluster, thus as by Claim \ref{claim:clustered3epsspanner}, $\dist_{H}(u,v)\le \dist_{G}(u,v)+2\cdot r_{T}$. Thus as in the proof of Lemma \ref{lem:3plusepsspanner}, for any $1\le d \le 4\cdot r_{T}$, we have that $\dist_{H}(u,v)\le (3+\epsilon)\cdot \dist_{G}(u,v)+4\cdot r_{T}$. Thus for any pair at distance $d$ we have:
\begin{equation*}
\dist_{H}(u,v)\le \lceil \frac{\dist_{G}(u,v)}{4\cdot r_{T}}\rceil \cdot ((3+\epsilon)\cdot 4\cdot r_{T} +4\cdot r_{T})\le (4+\epsilon)\cdot \dist_{G}(u,v)+(16+4\cdot\epsilon)\cdot r_{T}
\end{equation*}
\end{proof}
We now bound the round complexity in each phase $1\le i\le T$. Note that in the first stage of the algorithm we run a BFS traversal from all the cluster centers to a depth of $r_{i-1}+\alpha_i$. Since these traversals are node-disjoint, the round complexity of this stage is $O(r_{i-1}+\alpha_{i})=O(r_{i})$, thus over all $T$ phases the round complexity of this stage is $O(\sum_{i=1}^{T}r_{i})=O(\sum_{i=1}^{T}\left(5+16/\epsilon \right)^{i-1})=O(\beta)$. In the second stage we also run node-disjoint BFS traversals. The traversals are dont to the depth of $4\cdot r_{i-1}+4\cdot \alpha_{i}$, thus the round complexity of the second stage is also $O(\beta)$. In the third stage non-disjoint BFS traversals to a depth of $2\cdot r_{i-1}+2\cdot \alpha_{i}$ are made. By combining Chernoff Bound with Lemma \ref{lem:numberofbfstaversals} it holds that w.h.p each vertex is traversed by $\widetilde{O}(1/p_{i})=\widetilde{O}(1/p_{i_{0}})=\widetilde{O}(n^{\rho})$ vertices, thus in the \local\ model this stage takes  $\widetilde{O}(r_{i})$ and in the \congest\ model it takes $\widetilde{O}(n^{\rho}\cdot r_{i})$. Thus over all the algorithm run in $\widetilde{O}(\beta)$ rounds in the \local\ model and in $\widetilde{O}(n^{\rho}\cdot \beta)$ rounds in the \congest\ model.
\end{proof}

